HotStuff: BFT Consensus in the Lens of Blockchain

We present HotStuff, a leader-based Byzantine fault-tolerant replication protocol for the partially synchronous model. Once network communication becomes synchronous, HotStuff enables a correct leader to drive the protocol to consensus at the pace of actual (vs. maximum) network delay--a property called responsiveness--and with communication complexity that is linear in the number of replicas. To our knowledge, HotStuff is the first partially synchronous BFT replication protocol exhibiting these combined properties. HotStuff is built around a novel framework that forms a bridge between classical BFT foundations and blockchains. It allows the expression of other known protocols (DLS, PBFT, Tendermint, Casper), and ours, in a common framework. Our deployment of HotStuff over a network with over 100 replicas achieves throughput and latency comparable to that of BFT-SMaRt, while enjoying linear communication footprint during leader failover (vs. quadratic with BFT-SMaRt).

==> Makefile <==
.PHONY: all

LATEX=TZ='UTC' pdflatex
BIBTEX=bibtex
BIBFILE=paper.bib
PAPER=arxiv.pdf

ifeq ($(SUBMIT),yes)
	PREFIX='\def\submission{}\input{'
	SUFFIX='}'
else
	PREFIX=''
	SUFFIX=''
endif

TEXFILES = $(wildcard *.tex) $(wildcard sections/*.tex) $(wildcard figures/*.tex) $(wildcard figures/*.pdf)

all: $(PAPER)

%.pdf: %.tex $(BIBFILE) $(TEXFILES)
	$(LATEX) $(PREFIX)$<$(SUFFIX)
	$(BIBTEX) $(basename $@)
	$(LATEX) $(PREFIX)$<$(SUFFIX)
	$(LATEX) $(PREFIX)$<$(SUFFIX)

clean:
	rm -f *.aux *.log *~ *.out .DS_Store *.dvi $(PAPER) \
		*.lot *.lof *.toc *.blg *.bbl *.ent *.bak *.glo *.gls *.ist


==> podc2019-final/Makefile <==
.PHONY: all

LATEX=TZ='UTC' pdflatex
BIBTEX=bibtex
BIBFILE=paper.bib
PAPER=podc.pdf

ifeq ($(SUBMIT),yes)
	PREFIX='\def\submission{}\input{'
	SUFFIX='}'
else
	PREFIX=''
	SUFFIX=''
endif

TEXFILES = $(wildcard *.tex) $(wildcard sections/*.tex) $(wildcard figures/*.tex) $(wildcard figures/*.pdf)

all: $(PAPER)

%.pdf: %.tex $(BIBFILE) $(TEXFILES)
	$(LATEX) $(PREFIX)$<$(SUFFIX)
	$(BIBTEX) $(basename $@)
	$(LATEX) $(PREFIX)$<$(SUFFIX)
	$(LATEX) $(PREFIX)$<$(SUFFIX)

clean:
	rm -f *.aux *.log *~ *.out .DS_Store *.dvi $(PAPER) \
		*.lot *.lof *.toc *.blg *.bbl *.ent *.bak *.glo *.gls *.ist


==> podc2019-final/conclusion.tex <==
\section{Conclusion}

Since the introduction of PBFT, the first practical BFT replication solution in
the partial synchrony model,
numerous BFT solutions were built around its core two-phase paradigm. 
The first
phase guarantees proposal uniqueness through a \QC. The second phase guarantees
that a new leader can convince replicas to vote for a safe proposal. This
requires the leader to relay information from $(n-f)$ replicas, each reporting
its own highest \QC\ or vote. Generations of two-phase works thus suffer from a
quadratic communication bottleneck on leader replacement.

\HotStuff\ revolves around a three-phase core, allowing a new leader to simply
pick the highest \QC\ it knows of. This alleviates the above complexity
and at the same time considerably simplifies the leader replacement protocol.
Having (almost) canonized the phases, it is very easy to pipeline \HotStuff, and
to frequently rotate leaders. 


==> podc2019-final/evaluation.tex <==
\section{Evaluation}\label{app:eval}

We have implemented \multiversions{\HotStuffPro}{\HotStuff} as a library in roughly 4K
lines of C++ code. Most noticeably, the core consensus logic specified
in the pseudocode consumes only around 200 lines.
%Thanks to the notion of a \Gadget, we decouple safety and liveness handling entirely, simplifying each.
In this section, we will first examine baseline
throughput and latency by comparing to a state-of-art system,
BFT-SMaRt~\cite{BFTSMaRt}.  We then focus on the message cost for view
changes to see our advantages in this scenario.
 
\subsection{Setup}
We conducted our experiments on Amazon EC2 using \texttt{c5.4xlarge}
instances.  Each instance had 16 vCPUs supported by Intel Xeon
Platinum 8000 processors.  All cores sustained a Turbo CPU clock speed
up to 3.4GHz. We ran each replica on a single VM instance, and so
BFT-SMaRt, which makes heavy use of threads, was allowed to utilize 16
cores per replica, as in their original evaluation~\cite{BFTSMaRt}.
The network bandwidth on each machine was 3500Mbps, and we did not
limit bandwidth in any runs of either system.

Our prototype implementation of \HotStuff uses secp256k1 for all
digital signatures in both votes and quorum certificates. BFT-SMaRt
uses hmac-sha1 for MACs (Message Authentication Codes) in the messages
during normal operation and uses digital signatures in addition to
MACs during a view change.
 
All results for \HotStuff reflect end-to-end measurement from the
clients. For BFT-SMaRt, we used the micro-benchmark programs
\texttt{Throughput\-Latency\-Server} and
\texttt{Throughput\-Latency\-Client} from the BFT-SMaRt website
(\url{https://github.com/bft-smart/library}). The client program
measures end-to-end latency but not throughput, while the server-side
program measures both throughput and latency. We used the throughput
results from servers and the latency results from clients.
 
\subsection{Base Performance}
We first measured throughput and latency in a setting commonly seen in
the evaluation of other BFT replication systems. We ran 4 replicas in
a configuration that tolerates a single failure, i.e., $f = 1$, while
varying the operation request rate until the system saturated.  This
benchmark used empty (zero-sized) operation requests and responses and
triggered no view changes; we expand to other settings below.

\begin{figure}
    \includegraphics[width=\linewidth]{../graphs/thr-lat-1-hs.pdf}
    \captionof{figure}{Throughput vs.\@ latency with different choices of batch size, 4 replicas, 0/0 payload.}\label{fig:thr-lat1}
\end{figure}
\begin{figure}
    \includegraphics[width=\linewidth]{../graphs/thr-lat-2-hs.pdf}
    \captionof{figure}{Throughput vs.\@ latency with different choices of payload size with 4 replicas, batch size 400.}\label{fig:thr-lat2}
\end{figure}

Figure~\ref{fig:thr-lat1} depicts three batch sizes for both systems,
100, 400, and 800, though because these systems have different
batching schemes, these numbers mean slightly different things for
each system.  BFT-SMaRt drives a separate consensus decision for each
operation, and batches the messages from multiple consensus protocols.
Therefore, it has a typical L-shaped latency/throughput performance
curve.  \HotStuff batches multiple operations in each node, and in
this way, mitigates the cost of digital signatures per
decision. However, above $400$ operations per batch, the latency
incurred by batching becomes higher than the cost of the crypto.
Despite these differences, \HotStuff achieves comparable performance
to BFT-SMaRt for all three batch sizes.

For batch sizes of 100 and 400, the lowest-latency \HotStuff point
provides latency and throughput that are comparable to the latency and
throughput simultaneously achievable by BFT-SMaRT at its highest
throughput.  Recall that \HotStuff makes use of the first phase of
the next decision to piggyback the final phase of the previous one,
and so requires a moderate rate of submitted operations to achieve its
lowest-latency point.  Or, in other words, reducing the rate of
submitted operations further only \textit{increases} latency.  In
practice, this operation rate could be ensured by generating dummy
nodes to finalize a decision when there are insufficient outstanding
operations to do so naturally.  However, for these runs we did not
generate dummy nodes, but instead just ensured that operations were
submitted at rate sufficient to demonstrate low latency, which also
happened to roughly maximize throughput, as well.

Figure~\ref{fig:thr-lat2} depicts three client request/reply payload
sizes (in bytes) of 0/0, 128/128, and 1024/1024, designated by
``\verb|p0|'', ``\verb|p128|'', and ``\verb|p1024|''.  At payload size
of 1024 bytes, the reduced communication complexity of \HotStuff due
to its linear protocol and use of signatures already (slightly)
outperforms BFT-SMaRt.

Below we evaluate both systems in more challenging situations, where the
performance advantages of \HotStuff will become more pronounced. 

\subsection{Scalability}

To evaluate the scalability of \HotStuff in various dimensions, we
performed three experiments. For the baseline, we used zero-size
request/response payloads while varying the number of replicas.  The
second evaluation repeated the baseline experiment with 1024-byte
request/response payloads.  The third test repeated the baseline (with
empty payloads) while introducing network delays between replicas
that were uniformly distributed in 5ms $\pm$ 0.5ms or in 10ms $\pm$
1.0ms, implemented using \verb|NetEm| (see
\url{https://www.linux.org/docs/man8/tc-netem.html}).

The first setting is depicted as the ``\verb|p0|'' curves in
Figure~\ref{fig:n-thr-1} (throughput) and Figure~\ref{fig:n-lat-1}
(latency).  BFT-SMaRt shows (slightly) better scaling in both measures
than \HotStuff. This is mainly due its faster MAC computations. In the
future, we plan to reduce the cryptographic computation overhead in
\HotStuff by using (i) a faster signature scheme and (ii) employing
threshold signatures.

The second setting with payload size 1024 bytes is denoted by
``\verb|p1024|'' in Figure~\ref{fig:n-thr-1} (throughput) and
Figure~\ref{fig:n-lat-1} (latency).  Due to its quadratic bandwidth
cost, BFT-SMaRt performed worse than \HotStuff in both.

The third setting is shown in Figure~\ref{fig:n-thr-2} (throughput)
and Figure~\ref{fig:n-lat-2} (latency) as ``\verb|5ms|'' or
``\verb|10ms|''.  Again, due to the larger use of communication in
BFT-SMaRt, \HotStuff consistently outperformed BFT-SMaRt in both
cases.

%\DM{shall we say: These preliminary micro-benchmarks, especially the third
%settings, indicate that \HotStuff will perform well under real workloads.  In the
%future, we plan to repeat the evaluation over wide-area settings.}

\begin{figure}
    \includegraphics[width=\linewidth]{../graphs/n-thr-base.pdf}
    \captionof{figure}{Throughput vs.\@ number of nodes with 0/0 payload, batch size of 400.}\label{fig:n-thr-0}
\end{figure}
\begin{figure}
    \includegraphics[width=\linewidth]{../graphs/n-lat-base.pdf}
    \captionof{figure}{Latency vs.\@ number of nodes with 0/0 payload, batch size of 400.}\label{fig:n-lat-0}
\end{figure}

\begin{figure}
    \includegraphics[width=\linewidth]{../graphs/n-thr-payload.pdf}
    \captionof{figure}{Throughput vs.\@ number of nodes with payload size 128/128, and 1024/1024.}\label{fig:n-thr-1}
\end{figure}

\begin{figure}
    \includegraphics[width=\linewidth]{../graphs/n-lat-payload.pdf}
    \captionof{figure}{Latency vs.\@ number of nodes with payload size 128/128, and 1024/1024.}\label{fig:n-lat-1}
\end{figure}

\begin{figure}
    \includegraphics[width=\linewidth]{../graphs/n-thr-netlat.pdf}
    \captionof{figure}{Throughput vs.\@ number of nodes with inter-replica latency 5ms and 10ms.}\label{fig:n-thr-2}
\end{figure}

\begin{figure}
    \includegraphics[width=\linewidth]{../graphs/n-lat-netlat.pdf}
    \captionof{figure}{Latency vs.\@ number of nodes with inter-replica latency 5ms $\pm$ 0.5ms or 10ms $\pm$ 1.0ms.}\label{fig:n-lat-2}
\end{figure}

\subsection{View Change}

To evaluate the communication complexity of
leader replacement, we counted the number of \emph{signature or MAC
verifications} performed within BFT-SMaRt's view-change protocol. 
Our evaluation strategy was as follows. We injected a view change into BFT-SMaRt every one
thousand nodes. We instrumented the BFT-SMaRt source code to count the number of verifications
upon receiving and processing messages within the view-change protocol. 
Beyond communication complexity, 
this measurement underscores the cryptographic computation load
associated with transferring these authenticated values. 

Figure~\ref{fig:n-nauth} shows the number of extra authenticators
(MACs or signatures) processed for each view change,
where ``extra'' is defined to be those authenticators that would not be sent if the leader remained stable.  Note that \multiversions{\HotStuffPro}{\HotStuff} has no ``extra'' authenticators by this definition, since the number of authenticators remains the same regardless of whether the leader stays the same or not.
The figure depicts separate counts for MACs and for signatures, and shows that
BFT-SMaRt uses super-linear numbers of both.  \HotStuff does not
require extra authenticators for view changes and so is omitted from
the graph.

Evaluating the real-time performance of leader replacement is tricky. 
First, BFT-SMaRt got stuck when triggering frequent view changes; our
authenticator-counting benchmark had to average over as many successful
view changes as possible before the system got stuck, repeating the experiment
many times. Second, the actual elapsed time for leader replacement depends
highly on timeout parameters
%, on the \Gadget, and on
and the leader-election
mechanism. It is therefore impossible to provide a meaningful comparison.

\begin{figure}[ht]
    \includegraphics[width=\linewidth]{../graphs/n-nauth.pdf}
    \captionof{figure}{Number of extra authenticators used for each BFT-SMaRt view change.}\label{fig:n-nauth}
\end{figure}


==> podc2019-final/setup.tex <==
\usepackage{cancel}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{bm}
\usepackage{dsfont}
\usepackage{bbding}
\usepackage{slantsc}
\usepackage{thmtools, thm-restate}
%\usepackage{mathrsfs}
\usepackage{tikz}
\usepackage{capt-of}
\usepackage{caption}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{paralist}
\usepackage{enumitem}
\usepackage{url}
\usepackage{xspace}
\usepackage{soul}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{pifont}
\usepackage{setspace}

\usetikzlibrary{shapes}
\usetikzlibrary{arrows}
\usetikzlibrary{calc}
\usetikzlibrary{shadows}

%%% Pseudocode Tweaks
\makeatletter
\algnewcommand{\LineComment}[1]{\Statex \hskip\ALG@thistlm {\color{gray}\textrm{// #1}}}
\makeatother
\algnewcommand{\SectionComment}[2]{\Statex {\color{#2}\(\triangleright\) \textrm{#1}}}
\renewcommand{\algorithmiccomment}[1]{\hfill {\color{gray}\textrm{// #1}}}
\algnewcommand{\InlineComment}[1]{{\hspace{0.5em}\color{gray}\textrm{// #1}}}
\algnewcommand{\Phase}[1]{\SectionComment{#1}{myorange}}
\MakeRobust{\Call}
\DeclareCaptionFormat{algor}{%
\hrulefill\par\offinterlineskip\vskip1pt%
\textbf{#1#2}#3\offinterlineskip\hrulefill}
\DeclareCaptionStyle{algori}{singlelinecheck=off,format=algor,labelsep=space}
\captionsetup[algorithm]{style=algori}

%%% Misc Tweaks
\makeatletter 
\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
{1.25ex \@plus1ex \@minus.2ex}%
{-1em}%
{\normalfont\normalsize\bfseries}}
\makeatother

%\setlength{\textfloatsep}{1ex}
\urlstyle{rm}
\renewcommand\ttdefault{cmtt}
\let\oldemptyset\emptyset
\let\emptyset\varnothing
\setlength{\abovecaptionskip}{3pt plus 1pt minus 1pt}
\newcommand{\cmark}{\ding{51}}
\newcommand{\sharedbase}{./podc2019-final}

% New definitions
\algnewcommand\algorithmicswitch{\textbf{switch}}
\algnewcommand\algorithmiccase{\textbf{case}}
\algnewcommand\algorithmicassert{\texttt{assert}}
\algnewcommand\Assert[1]{\State \algorithmicassert(#1)}%
% New "environments"
\algdef{SE}[SWITCH]{Switch}{EndSwitch}[1]{\algorithmicswitch\ #1\ \algorithmicdo}{\algorithmicend\ \algorithmicswitch}%
\algdef{SE}[CASE]{Case}{EndCase}[1]{\algorithmiccase\ #1}{\algorithmicend\ \algorithmiccase}%
\algtext*{EndSwitch}%
\algtext*{EndCase}%⇧
\algnewcommand\algorithmiccontinue{\textbf{continue}}
\algnewcommand\algorithmicbreak{\textbf{break}}
\algnewcommand\Continue{\algorithmiccontinue}
\algnewcommand\Break{\algorithmicbreak}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{conjecture}[theorem]{Conjecture}
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\newtheorem{notation}{Notation}
\setcounter{footnote}{1}

\algnewcommand{\IIf}[1]{\State\algorithmicif\ #1\ \algorithmicthen}
\algnewcommand{\EndIIf}{\unskip\ \algorithmicend\ \algorithmicif}

\DeclareMathOperator*{\argmax}{\arg\max} 
\DeclareMathOperator*{\argmin}{\arg\min} 

\usetikzlibrary{calc}

\definecolor{myblue}{HTML}{0072bd}
\definecolor{myorange}{HTML}{d95319}
\definecolor{mybrown}{HTML}{ad2c0a}

%%%% Old Notations (reuse as much as possible)

\newcommand{\acset}{V}
\newcommand{\acsetof}[1]{\acset[#1]}
\newcommand{\qcset}{\mathit{certs}}
\newcommand{\qcsetof}[1]{\qcset[#1]}

\newcommand{\Lvl}{b}
\newcommand{\lvl}{w}
\newcommand{\Lvlx}{b}
\newcommand{\Lvlxx}{b'}
\newcommand{\Lvlxxx}{b''}
\newcommand{\lvly}{w}
\newcommand{\lvlyy}{w'}
\newcommand{\lvlyyy}{w''}
\newcommand{\Lqc}{\Lvl_\mathit{lock}}
\newcommand{\Lnew}{\Lvl_\mathit{new}}
\newcommand{\Ltail}{\Lvl_\mathit{leaf}}
\newcommand{\proposemsg}[3]{\langle\mathrm{propose}, #1, #2, #3 \rangle}
\newcommand{\votemsg}[3]{\langle\mathrm{vote}, {#2}_{\sigma_{#1}}, #3 \rangle}
\newcommand{\votemsgsig}[4]{\langle\mathrm{vote}, {#2}_{\sigma_{#1}#4}, #3 \rangle}
\newcommand{\assign}{\gets}
\newcommand{\QCedge}{(\Leftarrow \land \gets)}
\newcommand{\qcedge}{\Leftarrow}
\newcommand{\pathfrom}{\stackrel{*}{\gets}}
\newcommand{\nopathfrom}{\stackrel{*}{\cancel{\gets}}}
\newcommand{\vheight}{\mathit{vheight}}
\newcommand{\nheight}{\mathit{nextHeight}}
\newcommand{\Lexec}{\Lvl_\mathit{exec}}
\newcommand{\Cmd}{\mathit{cmd}}

\ifdefined\submission
   \newcommand{\remark}[1]{}
\else
    \newcommand{\remark}[1]{#1}
\fi
\newcommand{\DM}[1]{{\remark{\color{orange}{\textbf{DM: } #1}}}}
\newcommand{\TY}[1]{{\remark{\color{blue}{\textbf{TY: } #1}}}}
\newcommand{\MKR}[1]{{\remark{\color{blue}{\textbf{MKR: } #1}}}}

%%%% HotStuff Names

\newcommand{\HotStuffBasic}{Basic \HotStuff}
\newcommand{\HotStuffPro}{Chained \HotStuff}
\newcommand{\HotStuffX}{Incumbent \HotStuff}
\newcommand{\Gadget}{Pacemaker\xspace}

%%%% New Notations for PODC

%% Crypto
\newcommand{\sigSign}[1]{\ensuremath{\mathit{sign}_{#1}}\xspace}
\newcommand{\sigVerify}[1]{\ensuremath{\mathit{verify}_{#1}}\xspace}
\newcommand{\tsigSign}[1]{\ensuremath{\mathit{tsign}_{#1}}\xspace}
\newcommand{\tsigCombine}{\ensuremath{\mathit{tcombine}}\xspace}
\newcommand{\tsigVerify}{\ensuremath{\mathit{tverify}}\xspace}
\newcommand{\sig}{\ensuremath{\sigma}\xspace}
\newcommand{\partialResult}[1]{\ensuremath{\rho}_{#1}\xspace}
\newcommand{\cryptoHashFn}{\ensuremath{h}\xspace}

%% Variable Names
\newcommand{\gViewNumber}{\mathit{curView}}
\newcommand{\gBranch}{\mathit{curProposal}}
\newcommand{\fViewNumber}[1]{{#1}\mathit{.viewNumber}}
\newcommand{\fBranch}[1]{{#1}\mathit{.node}}
\newcommand{\fType}[1]{{#1}\mathit{.type}}
\newcommand{\fCert}[1]{{#1}\mathit{.sig}}
\newcommand{\fHeight}[1]{{#1}\mathit{.height}}
\newcommand{\fJustify}[1]{{#1}\mathit{.justify}}
\newcommand{\fParent}[1]{{#1}\mathit{.parent}}
\newcommand{\fCmd}[1]{{#1}\mathit{.cmd}}

\newcommand{\msgViewNumber}[1]{\fViewNumber{#1}}
\newcommand{\msgType}[1]{\fType{#1}}
\newcommand{\msgBranch}[1]{\fBranch{#1}}
\newcommand{\msgQC}[1]{#1\mathit{.justify}}
\newcommand{\msgSig}[1]{#1\mathit{.partialSig}}

\newcommand{\bMsgViewNumber}[1]{\mathbf{#1}\mathit{.viewNumber}}
\newcommand{\bMsgType}[1]{\mathbf{{#1}.type}}
\newcommand{\bMsgBranch}[1]{\mathbf{{#1}.node}}
\newcommand{\bMsgQC}[1]{\mathbf{{#1}.justify}}

\newcommand{\msgQCViewNumber}[1]{\fViewNumber{\msgQC{#1}}}
\newcommand{\msgQCBranch}[1]{\fBranch{\msgQC{#1}}}
\newcommand{\msgQCType}[1]{\fType{\msgQC{#1}}}

\newcommand{\cmd}{\mathit{cmd}}
\newcommand{\type}{\mathit{type}}
\newcommand{\branch}{\mathit{node}}
\newcommand{\parent}{\mathit{parent}}
\newcommand{\height}{\mathit{height}}
\newcommand{\viewNumber}{\mathit{viewNumber}}
%\newcommand{\qcVar}[1]{\mathit{#1}\mbox{-}\allowbreak{}\mathit{QC}}
\newcommand{\qcVar}[1]{\mathit{#1}\mathit{QC}}
\newcommand{\qc}{\mathit{qc}}
\newcommand{\Hqc}{\qc_{\mathit{high}}}
\newcommand{\justify}{\mathit{justify}}
\newcommand{\hqc}{\qcVar{high}}
\newcommand{\lqc}{\qcVar{locked}}
\newcommand{\prepareQC}{\qcVar{prepare}}
\newcommand{\keyQC}{\qcVar{precommit}}
\newcommand{\commitQC}{\qcVar{commit}}
\newcommand{\decideQC}{\qcVar{decide}}
\newcommand{\genericQC}{\qcVar{generic}}

%% Phase/concept Names
\newcommand{\PREPARE}{\textsc{prepare}\xspace}
\newcommand{\COMMIT}{\textsc{commit}\xspace}
\newcommand{\KEY}{\textsc{pre-commit}\xspace}
\newcommand{\DECIDE}{\textsc{decide}\xspace}
\newcommand{\NEWVIEW}{\textsc{new-view}\xspace}
\newcommand{\GENERIC}{\textsc{generic}\xspace}

\newcommand{\QC}{QC\xspace}
\newcommand{\QCfull}{quorum certificate\xspace}
\newcommand{\QCFull}{Quorum certificate\xspace}
\newcommand{\QCFULL}{Quorum Certificate\xspace}

\algnewcommand{\leader}{\Call{leader}{\gViewNumber}}
\algnewcommand{\nextLeader}{\Call{leader}{\gViewNumber+1}}
\algnewcommand{\leaderOf}[1]{\Call{leader}{#1}}

\algblock{As}{EndAs}
\algnewcommand\algorithmicas{\textbf{as}}
\algrenewtext{As}[1]{\algorithmicas\ #1}
\algtext*{EndAs}

